Do I Need the Cloud? Uncertainty-Aware Step-Level Handoff for Small Language Model Agents

Small language models (SLMs) are attractive as local agent controllers because they reduce remote inference, latency, and deployment footprint, yet structured tool errors can cause an agent step to fail. Existing routers typically select a model once per query. However, agents expose sequential decision points whose difficulty dynamically changes based on intermediate observations. We propose STEPGATE, an uncertainty-aware handoff framework that scores each local SLM action and selectively escalates challenging steps to a stronger model. On a 52-task held-out single-step BFCL-derived test split, the Qwen2.5-1.5B/7B pair attains 82.7% task success with 30.8% escalation, versus 67.3% local-only and 75.4% random escalation (which uses 33.8% escalation). In a separate multi-turn evaluation, STEPGATE achieves 69.0% trajectory success and 84.0% action success using only 30.0% cloud actions, compared with 48.0%/70.5% local-only, 60.0%/78.2% random escalation, and 57.0%/77.1% query-level routing (strong-only achieves 82.0% trajectory success at 100% cloud actions). These results suggest that step-level escalation recovers a large share of the performance gap to the stronger Qwen2.5-7B backend at a matched cloud-action rate while transmitting fewer tokens remotely. However, our evaluation is limited to one model family, a single stronger backend, and scripted tasks. Furthermore, the test sets are small, multi-turn comparisons rely on paired intervals and statistical tests, and our risk tiers serve as research annotations rather than formal safety guarantees.

==> tables/ablation_filled.tex <==
\begin{table}[b]
\centering\small
\caption{Ablation of the calibrated failure predictor (logistic regression), qwen2.5-1.5b, real BFCL subset (n=52 test tasks). Cloud budget fixed at 30\% (threshold chosen on calibration split only).}
\label{tab:ablation}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccc}
\toprule
Gate features & AUROC $\uparrow$ & ECE $\downarrow$ & Task succ. $\uparrow$ & Cloud \%\\
\midrule
All (\method) & 0.829 & 0.212 & 82.7 & 30.8\\
$-$ consistency & 0.832 & 0.231 & 82.7 & 28.8\\
$-$ schema/arguments & 0.829 & 0.241 & 82.7 & 30.8\\
$-$ risk & 0.886 & 0.119 & 86.5 & 34.6\\
Token uncertainty only & 0.565 & 0.078 & 76.9 & 28.8\\
\bottomrule
\end{tabular}
\end{table}

==> tables/ablations.tex <==
\begin{tabular}{llll rr}
\toprule
SLM & Feature set & Classifier & Status & AUROC & AUPRC \\
\midrule
qwen2.5-0.5b & full & logistic regression & OK & 0.729 & 0.777 \\
qwen2.5-0.5b & full & gradient boosted trees & OK & 0.679 & 0.569 \\
qwen2.5-0.5b & minus token uncertainty & logistic regression & OK & 0.770 & 0.768 \\
qwen2.5-0.5b & minus token uncertainty & gradient boosted trees & OK & 0.717 & 0.713 \\
qwen2.5-0.5b & minus schema & logistic regression & OK & 0.684 & 0.713 \\
qwen2.5-0.5b & minus schema & gradient boosted trees & OK & 0.648 & 0.545 \\
qwen2.5-0.5b & minus self consistency & logistic regression & OK & 0.685 & 0.756 \\
qwen2.5-0.5b & minus self consistency & gradient boosted trees & OK & 0.747 & 0.677 \\
qwen2.5-0.5b & minus risk metadata & logistic regression & OK & 0.784 & 0.810 \\
qwen2.5-0.5b & minus risk metadata & gradient boosted trees & OK & 0.733 & 0.654 \\
qwen2.5-0.5b & cheap only & logistic regression & OK & 0.685 & 0.756 \\
qwen2.5-0.5b & cheap only & gradient boosted trees & OK & 0.747 & 0.677 \\
qwen2.5-1.5b & full & logistic regression & OK & 0.829 & 0.832 \\
qwen2.5-1.5b & full & gradient boosted trees & OK & 0.854 & 0.819 \\
qwen2.5-1.5b & minus token uncertainty & logistic regression & OK & 0.804 & 0.803 \\
qwen2.5-1.5b & minus token uncertainty & gradient boosted trees & OK & 0.759 & 0.766 \\
qwen2.5-1.5b & minus schema & logistic regression & OK & 0.829 & 0.832 \\
qwen2.5-1.5b & minus schema & gradient boosted trees & OK & 0.854 & 0.819 \\
qwen2.5-1.5b & minus self consistency & logistic regression & OK & 0.832 & 0.838 \\
qwen2.5-1.5b & minus self consistency & gradient boosted trees & OK & 0.854 & 0.819 \\
qwen2.5-1.5b & minus risk metadata & logistic regression & OK & 0.886 & 0.841 \\
qwen2.5-1.5b & minus risk metadata & gradient boosted trees & OK & 0.830 & 0.817 \\
qwen2.5-1.5b & cheap only & logistic regression & OK & 0.832 & 0.838 \\
qwen2.5-1.5b & cheap only & gradient boosted trees & OK & 0.854 & 0.819 \\
qwen2.5-3b & full & logistic regression & OK & 0.899 & 0.735 \\
qwen2.5-3b & full & gradient boosted trees & OK & 0.851 & 0.419 \\
qwen2.5-3b & minus token uncertainty & logistic regression & OK & 0.830 & 0.511 \\
qwen2.5-3b & minus token uncertainty & gradient boosted trees & OK & 0.844 & 0.514 \\
qwen2.5-3b & minus schema & logistic regression & OK & 0.899 & 0.735 \\
qwen2.5-3b & minus schema & gradient boosted trees & OK & 0.822 & 0.474 \\
qwen2.5-3b & minus self consistency & logistic regression & OK & 0.899 & 0.717 \\
qwen2.5-3b & minus self consistency & gradient boosted trees & OK & 0.857 & 0.469 \\
qwen2.5-3b & minus risk metadata & logistic regression & OK & 0.880 & 0.514 \\
qwen2.5-3b & minus risk metadata & gradient boosted trees & OK & 0.855 & 0.397 \\
qwen2.5-3b & cheap only & logistic regression & OK & 0.899 & 0.717 \\
qwen2.5-3b & cheap only & gradient boosted trees & OK & 0.857 & 0.469 \\
\bottomrule
\end{tabular}

==> tables/calibration.tex <==
\begin{tabular}{lll rrrr}
\toprule
SLM & Feature set & Classifier & AUROC & AUPRC & Brier & ECE \\
\midrule
qwen2.5-0.5b & full & logistic regression & 0.729 & 0.777 & 0.203 & 0.154 \\
qwen2.5-0.5b & full & gradient boosted trees & 0.679 & 0.569 & 0.242 & 0.140 \\
qwen2.5-0.5b & minus token uncertainty & logistic regression & 0.770 & 0.768 & 0.194 & 0.113 \\
qwen2.5-0.5b & minus token uncertainty & gradient boosted trees & 0.717 & 0.713 & 0.241 & 0.232 \\
qwen2.5-0.5b & minus schema & logistic regression & 0.684 & 0.713 & 0.231 & 0.180 \\
qwen2.5-0.5b & minus schema & gradient boosted trees & 0.648 & 0.545 & 0.244 & 0.156 \\
qwen2.5-0.5b & minus self consistency & logistic regression & 0.685 & 0.756 & 0.211 & 0.148 \\
qwen2.5-0.5b & minus self consistency & gradient boosted trees & 0.747 & 0.677 & 0.235 & 0.177 \\
qwen2.5-0.5b & minus risk metadata & logistic regression & 0.784 & 0.810 & 0.203 & 0.140 \\
qwen2.5-0.5b & minus risk metadata & gradient boosted trees & 0.733 & 0.654 & 0.236 & 0.090 \\
qwen2.5-0.5b & cheap only & logistic regression & 0.685 & 0.756 & 0.211 & 0.148 \\
qwen2.5-0.5b & cheap only & gradient boosted trees & 0.747 & 0.677 & 0.235 & 0.177 \\
qwen2.5-1.5b & full & logistic regression & 0.829 & 0.832 & 0.144 & 0.212 \\
qwen2.5-1.5b & full & gradient boosted trees & 0.854 & 0.819 & 0.169 & 0.121 \\
qwen2.5-1.5b & minus token uncertainty & logistic regression & 0.804 & 0.803 & 0.156 & 0.238 \\
qwen2.5-1.5b & minus token uncertainty & gradient boosted trees & 0.759 & 0.766 & 0.176 & 0.143 \\
qwen2.5-1.5b & minus schema & logistic regression & 0.829 & 0.832 & 0.147 & 0.241 \\
qwen2.5-1.5b & minus schema & gradient boosted trees & 0.854 & 0.819 & 0.169 & 0.121 \\
qwen2.5-1.5b & minus self consistency & logistic regression & 0.832 & 0.838 & 0.147 & 0.231 \\
qwen2.5-1.5b & minus self consistency & gradient boosted trees & 0.854 & 0.819 & 0.169 & 0.121 \\
qwen2.5-1.5b & minus risk metadata & logistic regression & 0.886 & 0.841 & 0.130 & 0.119 \\
qwen2.5-1.5b & minus risk metadata & gradient boosted trees & 0.830 & 0.817 & 0.134 & 0.120 \\
qwen2.5-1.5b & cheap only & logistic regression & 0.832 & 0.838 & 0.147 & 0.231 \\
qwen2.5-1.5b & cheap only & gradient boosted trees & 0.854 & 0.819 & 0.169 & 0.121 \\
qwen2.5-3b & full & logistic regression & 0.899 & 0.735 & 0.075 & 0.135 \\
qwen2.5-3b & full & gradient boosted trees & 0.851 & 0.419 & 0.100 & 0.137 \\
qwen2.5-3b & minus token uncertainty & logistic regression & 0.830 & 0.511 & 0.141 & 0.228 \\
qwen2.5-3b & minus token uncertainty & gradient boosted trees & 0.844 & 0.514 & 0.140 & 0.253 \\
qwen2.5-3b & minus schema & logistic regression & 0.899 & 0.735 & 0.081 & 0.144 \\
qwen2.5-3b & minus schema & gradient boosted trees & 0.822 & 0.474 & 0.097 & 0.154 \\
qwen2.5-3b & minus self consistency & logistic regression & 0.899 & 0.717 & 0.077 & 0.127 \\
qwen2.5-3b & minus self consistency & gradient boosted trees & 0.857 & 0.469 & 0.101 & 0.115 \\
qwen2.5-3b & minus risk metadata & logistic regression & 0.880 & 0.514 & 0.090 & 0.118 \\
qwen2.5-3b & minus risk metadata & gradient boosted trees & 0.855 & 0.397 & 0.103 & 0.164 \\
qwen2.5-3b & cheap only & logistic regression & 0.899 & 0.717 & 0.077 & 0.127 \\
qwen2.5-3b & cheap only & gradient boosted trees & 0.857 & 0.469 & 0.101 & 0.115 \\
\bottomrule
\end{tabular}

==> tables/main_filled.tex <==
\begin{table}[t]
\centering\small
\caption{Main results, qwen2.5-1.5b (local) / qwen2.5-7b 4-bit (strong), real 100-task BFCL subset, 52 test tasks. Cloud rate budget-matched at 30\% target (threshold/model chosen on calibration split only, applied once to test). ``Wrong risky'' = \% of executed test actions that were both incorrect and risk-tier $\geq$R2 (our taxonomy has no R3 action type in this task set).}
\label{tab:main}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc}
\toprule
System & Task succ. $\uparrow$ & Cloud \% $\downarrow$ & Wrong risky $\downarrow$ & Latency $\downarrow$ & Remote tok. $\downarrow$\\
\midrule
SLM only & 67.3 & 0 & 15.4 & 0.702 & 0\\
Strong only & 92.3 & 100 & 3.8 & 2.255 & 475.0\\
Random @ budget & 75.4 & 33.8 & 10.8 & 0.823 & 158.5\\
Query-level router & 73.1 & 42.3 & 15.4 & 1.052 & 266.2\\
Self-consistency & 82.7 & 38.5 & 7.7 & 0.829 & 175.2\\
\textbf{\method} & 82.7 & 30.8 & 3.8 & 0.777 & 134.5\\
\bottomrule
\end{tabular}
\end{table}

==> tables/main_results.tex <==
\begin{tabular}{llrrr}
\toprule
SLM & Method & Task success (\%) & 95\% CI & Escalation (\%) \\
\midrule
qwen2.5-0.5b & always local & 55.8 & [42.3, 69.2] & 0.0 \\
qwen2.5-0.5b & always strong & 92.3 & [84.6, 98.1] & 100.0 \\
qwen2.5-0.5b & oracle nondeployable & 94.2 & [86.5, 100.0] & 38.5 \\
qwen2.5-0.5b & entropy threshold@50pct & 76.9 & [65.4, 88.5] & 44.2 \\
qwen2.5-0.5b & self consistency threshold@50pct & 92.3 & [84.6, 98.1] & 100.0 \\
qwen2.5-0.5b & learned gate logistic regression@50pct & 78.8 & [67.3, 90.4] & 51.9 \\
qwen2.5-0.5b & learned gate gradient boosted trees@50pct & 80.8 & [69.2, 90.4] & 48.1 \\
qwen2.5-0.5b & random budget matched avg5seeds & 77.3 & [73.1, 82.7] & 51.9 \\
qwen2.5-1.5b & always local & 67.3 & [53.8, 80.8] & 0.0 \\
qwen2.5-1.5b & always strong & 92.3 & [84.6, 98.1] & 100.0 \\
qwen2.5-1.5b & oracle nondeployable & 94.2 & [88.5, 100.0] & 26.9 \\
qwen2.5-1.5b & entropy threshold@50pct & 84.6 & [75.0, 94.2] & 46.2 \\
qwen2.5-1.5b & self consistency threshold@50pct & 92.3 & [84.6, 98.1] & 100.0 \\
qwen2.5-1.5b & learned gate logistic regression@50pct & 84.6 & [75.0, 94.2] & 44.2 \\
qwen2.5-1.5b & learned gate gradient boosted trees@50pct & 88.5 & [78.8, 96.2] & 71.2 \\
qwen2.5-1.5b & random budget matched avg5seeds & 78.8 & [71.2, 84.6] & 44.2 \\
qwen2.5-3b & always local & 88.5 & [78.8, 96.2] & 0.0 \\
qwen2.5-3b & always strong & 92.3 & [84.6, 98.1] & 100.0 \\
qwen2.5-3b & oracle nondeployable & 94.2 & [88.5, 100.0] & 5.8 \\
qwen2.5-3b & entropy threshold@50pct & 90.4 & [80.8, 98.1] & 30.8 \\
qwen2.5-3b & self consistency threshold@50pct & 92.3 & [84.6, 98.1] & 100.0 \\
qwen2.5-3b & learned gate logistic regression@50pct & 90.4 & [80.8, 98.1] & 42.3 \\
qwen2.5-3b & learned gate gradient boosted trees@50pct & 90.4 & [80.8, 98.1] & 28.8 \\
qwen2.5-3b & random budget matched avg5seeds & 90.8 & [88.5, 94.2] & 42.3 \\
\bottomrule
\end{tabular}
